Three Decades of Deception Techniques in Active Cyber Defense -- Retrospect and Outlook

Deception techniques have been widely seen as a game changer in cyber defense. In this paper, we review representative techniques in honeypots, honeytokens, and moving target defense, spanning from the late 1980s to the year 2021. Techniques from these three domains complement with each other and may be leveraged to build a holistic deception based defense. However, to the best of our knowledge, there has not been a work that provides a systematic retrospect of these three domains all together and investigates their integrated usage for orchestrated deceptions. Our paper aims to fill this gap. By utilizing a tailored cyber kill chain model which can reflect the current threat landscape and a four-layer deception stack, a two-dimensional taxonomy is developed, based on which the deception techniques are classified. The taxonomy literally answers which phases of a cyber attack campaign the techniques can disrupt and which layers of the deception stack they belong to. Cyber defenders may use the taxonomy as a reference to design an organized and comprehensive deception plan, or to prioritize deception efforts for a budget conscious solution. We also discuss two important points for achieving active and resilient cyber defense, namely deception in depth and deception lifecycle, where several notable proposals are illustrated. Finally, some outlooks on future research directions are presented, including dynamic integration of different deception techniques, quantified deception effects and deception operation cost, hardware-supported deception techniques, as well as techniques developed based on better understanding of the human element.

==> sections/conclusion.tex <==

%In this paper, we did a survey of publicly released Android exploits and proposed a taxonomy of Android exploits from multiple perspectives by analyzing the collected real-world exploits and conducting an evaluation of these exploits on a set of devices.
%We analyzed the characteristics of each category and presented the trend view of the Android exploits along the timeline from the technical perspective based on the exploit data.
%We also shared our discussion and outlook gained from the observation of evaluation.


==> sections/exploit_table.tex <==
\afterpage{
	\onecolumn
	\small
	% Config the row spacing
	\def\arraystretch{1.25}
	% Config the column spacing
	\setlength{\tabcolsep}{1pt}
	\begin{landscape}
			
	\begin{longtable}{
		>{\centering\arraybackslash}p{0.6cm}
		>{\centering\arraybackslash}p{0.5cm}
		p{3.8cm}
		>{\centering\arraybackslash}p{3.1cm}
		>{\centering\arraybackslash}p{.8cm}
		>{\centering\arraybackslash}p{.8cm}
		>{\centering\arraybackslash}p{.8cm}
		>{\centering\arraybackslash}p{2.9cm}
		>{\centering\arraybackslash}p{3.6cm}
		>{\centering\arraybackslash}p{3.1cm}
		>{\centering\arraybackslash}p{2.8cm}
		>{\centering\arraybackslash}p{.3cm}
	}
	\caption{Survey Result of Android Exploits}\label{tab:all_exploits} \\
	\hline  
	\rowcolor[gray]{1.0}\textbf{Year} 
		& \multicolumn{2}{c}{\textbf{Exploit}} 
		& \textbf{Author}
		& \textbf{\rotatebox[origin=c]{270}{\makecell{Execution\\Channel\textsubscript{ 1}}}} 
		& \textbf{\rotatebox[origin=c]{270}{\makecell{Attack\\Vector\textsubscript{ 2}}}} 
		& \textbf{\rotatebox[origin=c]{270}{\makecell{\ Vulnerable\ \ \\Target\textsubscript{ 3}}}}
		& \textbf{Vulnablitiy (CVE)} 
		& \textbf{Vulnablity Type (CWE)}  
		& \textbf{\rotatebox[origin=c]{270}{\makecell{Target\\Devices}}} 
		& \textbf{\rotatebox[origin=c]{270}{\makecell{\ Affected\ \ \\\ Versions\ \ }}} 
		& \textbf{\rotatebox[origin=c]{270}{Verified}} \\\hline

	\endfirsthead	
	\multicolumn{3}{c}%
	{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \hline
	\hline
		\rowcolor[gray]{1.0} 
		\textbf{Year} 
		& \multicolumn{2}{c}{\textbf{Exploit}} 
		& \textbf{Author}
		& \textbf{\rotatebox[origin=c]{270}{\makecell{Exe.\\Channel}}} 
		& \textbf{\rotatebox[origin=c]{270}{\makecell{Attack\\Vector}}} 
		& \textbf{\rotatebox[origin=c]{270}{\makecell{Vul.\\Target}}}
		& \textbf{Vulnablitiy (CVE)} 
		& \textbf{Vulnablity Type (CWE)}
		& \textbf{\rotatebox[origin=c]{270}{\makecell{Target\\Devices}}} 
		& \textbf{\rotatebox[origin=c]{270}{\makecell{\ Affected\ \ \\\ Versions\ \ }}}
		& \textbf{\rotatebox[origin=c]{270}{Verified}} \\\hline
 
	\endhead		
	\multicolumn{3}{r}{\textbf{Continued on next page}} \\ \hline
	\endfoot
	\hline 
	\endlastfoot
	
	% Year 2009
	2009	& 1	& volez	& Christopher Lais (Zinx)	& O & O	& SYS	& N.A.	& N.A.	& Motorola Droid	& 2.0 and 2.0.1 	& -- \\ \hline
	
	% Year 2010	 
	2010	& 2	& exploid & Sebastian Krahmer	& S & M	& KRN	& CVE-2009-1185	& Input Validation (CWE-20)	& All	& Up to 2.3.4	& \checkmark \\ \cline{2-12}
	& 3	& RageAgainstTheCage 	& Sebastian Krahmer	& S & D	& SYS	& N.A.	& N.A.	& All	& Up to 2.2 	& \checkmark	\\ \cline{2-12}
	& 4	& Use-After-Free Remote Code Execution on Webkit	& Itzhak Avraham	& R & R,M	& SYS	& CVE-2010-1807	& Input Validation (CWE-20)	& Unspecified\textsuperscript{ 4}	& 2.0 to 2.1	& --	 \\ \cline{2-12}
	& 5	& Zimperlich / \newline zygote jailbreak	& Sebastian Krahmer	& S & D	& SYS	& N.A.	& N.A.	& All	& Up to 2.2 	& \checkmark	\\ \hline

	% Year 2011	 
	2011	& 6	& KillingInTheNameOf	& Sebastian Krahmer	& S & A	& SYS	& CVE-2011-1149	& Permissions, Privileges  and Access Control (CWE-264)	& All	& 2.1 to 2.2.2 	& \checkmark	\\ \cline{2-12}
	& 7	& psneuter ashmem exploit	& Scott Walker (scotty2)	& S & A	& SYS	& CVE-2011-1149	& Permissions, Privileges and Access Control (CWE-264)	& All	& Unspecified 	& \checkmark	\\ \cline{2-12}
	& 8	& levitator	& Jon Larimer and Jon Oberheide	& S & M	& VND	& CVE-2011-1350 CVE-2011-1352	& Information Leak / Disclosure (CWE-200) \newline Buffer Errors (CWE-119)	& Devices with the PowerVR SGX chipset	& 1.0 to 2.3.5 	& --	\\ \cline{2-12}
	& 9	& WebKit use-after-free	& MJ Keith	& R & R,M	& SYS	& CVE-2010-1119	& Resource Management Errors (CWE-399)	& Unspecified	& 2.0 to 2.1.1 	& --	\\ \cline{2-12}
	& 10	& Zysploit	& Joshua Wise (jwise)	& S & D	& SYS	& N.A.	& N.A.	& All	& Up to 2.2 	& \checkmark	\\ \cline{2-12}
	& 11	& GingerBreak	& Sebastian Krahmer	& A & M	& SYS	& CVE-2011-1823	& Numeric Errors (CWE-189)	& All	& 2.1 to 2.3.3, 3.0 	& --	\\ \cline{2-12}
	& 12	& sock\_sendpage local root / \newline asroot / Wunderbar	& Christopher Lais (Zinx)	& S & M	& KRN	& CVE-2009-2692	& Buffer Errors (CWE-119)	& All	& Up to 3.2.6 	& --	\\ \cline{2-12}
	& 13	& zergRush	& Revolutionary	& S & M	& SYS	& CVE-2011-3874	& Buffer Errors (CWE-119)	& All	& 2.2.x till 2.2.2, 2.3.x till 2.3.6	& -- \\ \cline{2-12}
	& 14	& TacoRoot	& Justin Case (jcase)	& S & P	& FLS	& N.A.	& N.A.	& EVO 4G and some other HTC models	& 2.x	& -- \\ \hline

	% Year 2012	 
	2012	& 15	& NachoRoot	& Justin Case (jcase)	& S & P	& FLS	& N.A.	& Permissions, Privileges and Access Control (CWE-264)	& ASUS Transformer Prime	& 4.0 to 4.0.4	& -- \\ \cline{2-12}
	& 16	& TPSparkyRoot	& sparkym3	& S & P	& FLS	& N.A.	& Permissions, Privileges and Access Control (CWE-264)	& ASUS Transformer Prime	& 4.0 to 4.0.4	& -- \\ \cline{2-12}
	& 17	& mempodroid / mempodipper / mem exploit	& Jay Freeman (saurik)	& S & P	& KRN	& CVE-2012-0056	& Permissions, Privileges and Access Control (CWE-264)	& Acer A200 Tablet, Galaxy Nexus, Motorola RAZR, Nexus S, Asus Transformer Prime	& 4.0.1 to 4.0.3	& -- \\ \cline{2-12}
	& 18	& Z2 Root Exploit	& Sacha (xsacha), cubundcube and Andreas Makris (bin4ry)	& S & D	& SYS	& N.A.	& N.A.	& Many Sony Xperia models, 3.x and 4.x before 4.1.1 & Unspecified & -- \\ \cline{2-12}
	& 19	& LG lit	& giantpune	& A & M	& VND	& CVE-2012-4220	& N.A.	& LG (with LM3530 backlight driver)	& Unspecified & -- \\ \cline{2-12}
	& 20	& Exynos Abuse / Sam (exynos-mem) Exploit	& alephzain	& S & M	& VND	& CVE-2012-6422	& Permissions, Privileges and Access Control (CWE-264)	& Samsung (Exynos 4 based)	& Unspecified	& \checkmark \\ \cline{2-12}
	& 21	& diaggetroot	& goroh kun	& A & M	& VND	& CVE-2012-4220	& 	& HTC J Butterfly	& Unspecified	& -- \\ \hline

	% Year 2013
	2013	& 22	& Qualcomm Gandalf camera driver exploit	& alephzain	& S & M	& VND	& CVE-2013-2595	& Permissions, Privileges and Access Control (CWE-264)	& Many models made by Asus, Huawei, LG etc.	& Unspecified	& \checkmark \\ \cline{2-12}
	& 23	& Motochopper / \newline fb\_mem\_exploit	& Dan Rosenberg (djrbliss)	& S & M	& KRN	& CVE-2013-2596	& Numeric Errors (CWE-189)	& Motorola (Atrix HD, Razr HD, Razr M) and other devices with Snapdragon S4 series	& Up to 4.2	& \checkmark \\ \cline{2-12}
	& 24	& libperf\_event	& Hiroyuki Ikezoe	& S & M	& KRN	& CVE-2013-2094	& Numeric Errors (CWE-189)	& Nexus 4 and Some Japanese models made by HTC, Fujitsu, Sharp, Sony and LG	& 4.0 to 4.3.1 (Linux Kernel version before 3.8.9)	&	\checkmark \\ \cline{2-12}
	& 25	& LG Sprite software backup / \newline LGPwn exploit	& Justin Case (jcase)	& A & P	& FLS	& CVE-2013-3685 (R)\textsuperscript{ 5}	& Race conditions	& 43 LG Optimus models	& Unspecified	&	-- \\ \cline{2-12}
	& 26	& libfj hdcp	& fi01	& S & M	& VND	& N.A.	& N.A.	& F05D, ISW11F and some other Docomo Fujitsu models	& Unspecified	&	-- \\ \cline{2-12}
	& 27	& Defy republic init\_runit	& Justin Case (jcase)	& S & M	& VND	& CVE-2013-4777 CVE-2013-5933	& Configuration (CWE-16) Buffer Errors (CWE-119)	& Motorola Defy XT 	& 2.3.7	&	-- \\ \cline{2-12}
	& 28	& libdiag Exploit 	& Hiroyuki Ikezoe	& S & M	& VND	& N.A.	& Input Validation (CWE-20)\newline Numeric Errors (CWE-189)	& Many models made by NEC, Fujitsu, etc	& Unspecified	&	-- \\ \cline{2-12}
	& 29	& Boromir (camera-isp) \newline exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Many models (MTK based)	& Unspecified	&	-- \\ \cline{2-12}
	& 30	& Gemli (dev/DspBridge)\newline exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Many models (TI OMAP 36XX based)	& Unspecified	&	-- \\ \cline{2-12}
	& 31	& Frodo (exynos-mem) exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Many models (Exynos based)	& Unspecified	&	-- \\ \cline{2-12}
	& 32	& Legolas (graphics/fb) exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Many models (Exynos based)	& Unspecified	&	-- \\ \cline{2-12}
	& 33	& Aragorn (video1) exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Many models (Exynos based)	& Unspecified	&	\checkmark \\ \cline{2-12}
	& 34	& Merry (s5p-smem) exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Many models (Exynos based)	& Unspecified	&	-- \\ \cline{2-12}
	& 35	& Android put\_user / get\_user \newline exploit \textit{(Metasploit module)}	& fi01, cubeundcube and timwr	& R & R,M	& KRN	& CVE-2013-6282	& Input Validation (CWE-20)	& Unspecified	& Linux kernel before 3.5.5 on the v6k and v7 ARM platforms, fixed in Jul 2013	&	\checkmark \\ \cline{2-12} 
	& 36	& TwerkMyMoto	& Justin Case (jcase)	& S & P	& FLS	& N.A.	& N.A.	& Motorola Razr I	& 4.1.2	& -- \\ \cline{2-12}
	& 37	& Pippin (memalloc) exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Many K3V2 based models made by Huawei	& Unspecified	&	-- \\ \cline{2-12}
	& 38	& Gollum (amjpegdec) exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Unspecified (AMLogic based)	& Unspecified	&	-- \\ \cline{2-12}
	& 39	& Faramir (camera-sysr) \newline exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Many models (MTK based)	& Unspecified	&	-- \\ \hline		
	
	% Year 2014		
	2014	& 40	& Barahir (Vcodec) exploit\textsuperscript{*}	& alephzain	& A & M	& VND	& N.A.	& N.A.	& Many models (MTK based)	& Unspecified	&	-- \\ \cline{2-12}
	& 41	& WeakSauce	& Justin Case (jcase) and Sean Beaupre (beaups)	& A & P	& FLS	& CVE-2014-3847 (R)	& N.A.	& HTC One m7, m7 on Verizon, m8 and Droid DNA	& 4.1 to 4.4.4	&	-- \\ \cline{2-12}
	& 42	& Qualcomm buffer overflow in acdb audio driver \newline (msm\_acdb\_exploit)	& fi01	& S & M	& VND	& CVE-2013-2597	& Buffer Errors (CWE-119)	& Unspecified	& Linux kernel 2.6.x - 3.x before Jun 2013	&	-- \\ \cline{2-12}
	& 43	& Pie / vold asec	& Justin Case (jcase)	& S & P	& SYS	& N.A.	& N.A.	& Moto X on locked carrier  	& 2.2.1 to 4.4.2	&	-- \\ \cline{2-12}
	& 44	& TowelRoot / futex exploit	& George Hotz (geohot)	& A & M	& KRN	& CVE-2014-3153	& Permissions, Privileges and Access Control (CWE-264)	& All	& Up to 4.4 ROMs built before Jun 2014	&	\checkmark \\ \cline{2-12}
	& 45	& StumpRoot	& IOMonster, Justin Case (jcase), autoprime and PlayfulGod	& A & O	& VND	& N.A.	& N.A.	& Many models made by LG	& Unspecified	&	-- \\ \cline{2-12}
	& 46	& Android Browser exploit \newline (ht\_webkit\_Android4)	& Hacking Team	& R & R,M	& SYS	& CVE-2011-1202 CVE-2012-2825 CVE-2012-2871	& Input Validation (CWE-20)	& Unspecified	& 4.0 to 4.3	&	-- \\ \hline
	
	% Year 2015
	2015	& 47	& ObjectInputStream local root	& Di Shen (retme7)	& A & M	& VND	& CVE-2014-4322 CVE-2014-7911	& N.A.	& Nexus 5	& 4.4.4	&	\checkmark \\ \cline{2-12}
	& 48	& libmsm memory corruption in camera driver \newline (libmsm\_vfe\_read\_exploit)	& Hiroyuki Ikezoe	& S & M	& VND	& CVE-2014-4321 (R) CVE-2014-4324 (R) CVE-2014-0975 (R) CVE-2014-0976 (R) CVE-2014-9409 (R)	& Input Validation (CWE-20)	& Unspecified	& Unspecified	&	-- \\ \cline{2-12}
	& 49	& PingPongRoot	&  Keen Team	& A & M	& KRN	& CVE-2015-3636	& Other (NVD-CWE-Other) \newline Uninitialized data structure	& Samsung Galaxy S6, Samsung Galaxy S6 Edge, HTC One (M9)	& 5.0 to 5.1.0	&	-- \\ \cline{2-12}
	& 50	& Mate7 TrustZone Exploit	& Di Shen (retme7)	& S & M	& TEE	& CVE-2015-4421 (R) CVE-2015-4422 (R)	& N.A.	& Huawei Mate7	& Unspecified	&	-- \\ \cline{2-12}
	& 51	& Mtkfb Exploit	& nforest@KeenTeam	& S & M	& VND	& N.A.	& N.A.	& Unspecified (MTK MT658X and MT6592 based)	& Unspecified	&	-- \\ \cline{2-12}
	& 52	& Full TrustZone exploit for \newline MSM8974	& laginimaineb	& S & M	& TEE	& N.A.	& N.A.	& Nexus 5	& A crafted ROM built based on 4.4.4	&	-- \\ \cline{2-12}
	& 53	& QSEECOM driver memory \newline corruption	& laginimaineb	& S & M	& TEE	& CVE-2014-4322	& Buffer Errors (CWE-119)	& Unspecified	& Unspecified	&	-- \\ \cline{2-12}
	& 54	& Stagefright Remote Code \newline Execution \newline \textit{(Metasploit module)}	& Joshua Drake (jduck) and NorthBit	& R & R,M	& SYS	& CVE-2015-1538 CVE-2015-1539 CVE-2015-3824 CVE-2015-3826 CVE-2015-3827 CVE-2015-3828 CVE-2015-3829	& Buffer Errors (CWE-119) \newline Numeric Errors (CWE-189)	& Nexus 5, Nexus 6, Nexus 7 and Samsung Galaxy S5 (SM-G900V)	& 5.0 to 5.1.1	&	\checkmark \\ \hline
		
	% Year 2016
	2016	& 55	& mediaserver code-exec	& laginimaineb	& S & M	& SYS	& CVE-2014-7920 (R) CVE-2014-7921 (R)	& Permissions, Privileges and Access Control (CWE-264)	& Unspecified	& 4.3 to 5.1	&	-- \\ \cline{2-12}
	& 56	& sensord local root	& s0m3b0dy	& S & M	& VND	& N.A.	& N.A.	& LG L7 and other devices have sensord deamon 	& Unspecified	&	-- \\ \cline{2-12}
	& 57	& Metaphor	& Hanan Beer@NorthBit	& R & R,M	& SYS	& CVE-2015-3864	& Numeric Errors (CWE-189)	& Nexus 5	& 5.0 to 5.1.1	&	-- \\ \cline{2-12}
	& 58	& iovyroot / pipe inatomic	& idl3r	& S & M	& KRN	& CVE-2015-1805	& Code (CWE-17)	& LG G Flex 2, many models made by Sony, Huawei and other brands	& 4.4.3 to 6.0	&	\checkmark \\ \cline{2-12}
	& 59	& Use-After-Free camera\newline driver exploit	& betalphafai (Edward Hung)	& S & M	& VND	& CVE-2015-0568	& Use After Free (CWE-416)	& Unspecified (Qualcomm MSM 7x30)	& Unspecified (Linux kernel 3.0.x)	&	-- \\ \cline{2-12}
	& 60	& QSEE TrustZone	& laginimaineb	& S & M	& TEE	& CVE-2015-6639	& Permissions, Privileges and Access Control (CWE-264)	& Nexus 6	& Unspecified	&	-- \\ \cline{2-12}
	& 61	& prctl\_vma\_exploit	& betalphafai (Edward Hung)	& S & M	& KRN	& CVE-2015-6640	& Permissions, Privileges and Access Control (CWE-264)	& Unspecified	& 5.1.1 and 6.0	&	\checkmark  \\ \cline{2-12}
	& 62	& Qualcomm TrustZone	& laginimaineb	& S & M	& TEE	&  CVE-2016-2431	& Permissions, Privileges and Access Control (CWE-264)	& Unspecified	& Unspecified	&	-- \\ \cline{2-12}
	& 63	& Dirty Cow (dirtyc0w)	& timwr	& S & M	& KRN	& CVE-2016-5195	& Race Condition (CWE-362)	& Unspecified	& Up to 7.0	&	-- \\  \hline	
	\end{longtable}
	% GRAND TABLE ENDS HERE
	\vspace{-1px}
	
	\textsuperscript{1} Legend for execution channels: (\underline{A}) App Execution Channel; (\underline{S}) Shell Execution Channel;
	(\underline{R}) Remote Execution Channel and (\underline{O}) notates Other Channels.
	\vspace{1px}
	
	\textsuperscript{2} Legend for attack vectors: (\underline{A}) Shared Memory (\texttt{ashmem}) Remapping; (\underline{D}) Daemon Abusing;
	(\underline{P}) File Permission \& Symbolic Link Attack; (\underline{M}) for Memory Corruption; 
	(\underline{R}) Remote Shell Control and (\underline{O}) Others.
	
	\vspace{1px}
	
	\textsuperscript{3} Legend for vulnerable targets: (\underline{FLS}) File System; (\underline{KRN}) Linux Kernel; 
	(\underline{SYS}) System, (\underline{TEE}) Trusted Execution Environment and (\underline{VND}) Vendor Drivers.
	\vspace{1px}
		
	\textsuperscript{4} The term ``Unspecific'' means the information has neither been disclosed by the author nor mentioned by any trusted source from Internet. 
	\vspace{1px}
	
	\textsuperscript{5} The annotation ``(R)'' after a CVE identifier represents as ``RESERVED'', which has been reserved for use by a CVE Numbering Authority (CNA) or researcher without all details being publicly disclosed.
	\vspace{1px}
		
	\textsuperscript{*} Discrete exploits integrated in \textit{framaroot} root application. Those exploits could be initiated by either running a shell command or app execution. 
	
	\vspace{1px}
	\begin{center}
		\textbf{End of table}
	\end{center}

	\end{landscape}
	\twocolumn
} % end of scope of "\afterpage" directive

